A Set-Based Approach for Robust Control Co-Design

Control Co-Design (CCD) considers the coupled effects of both the plant and control parameters to optimize a system's closed-loop transient performance during the design stage. This paper presents a new method for CCD with guarantees on robustness to nondeterministic disturbances for all initial conditions within a specified region of operation. This is accomplished by calculating the reachable sets of a candidate closed-loop system directly within the optimization problem. Using this approach, the plant and control parameters are simultaneously chosen to shape these reachable sets to be robustly positive invariant and thus safe for all time. Compared to conventional approaches that perform the optimization for a single initial condition and an a priori chosen sequence of disturbances, the proposed set-based method avoids sensitivity to variations in the assumed design scenario. As a representative example, the proposed method is applied to an active suspension system.

==> 05_CaseStudy.tex <==
\section{Case Study: TMS with TES}\label{sec-caseStudy}

This section applies the proposed set-based rCCD approach to a Thermal Management System (TMS) with an integrated Thermal Energy Storage (TES) module storing thermal energy as latent heat within a Phase Change Material (PCM) as depicted in Figure \ref{fig-TMS_Diagram}. The goal of the co-design problem is to choose the capacitance of the heat exchanger, phase change material, and volume of the fluid tank as well as a control policy to guarantee that temperature constraints are never violated for a bounded sequence of heat loads while minimizing the total system mass. 

\begin{figure}[!htb]
     \centering
     \includegraphics[width=1\linewidth]{figures/TMS_Diagram.pdf}
     \caption{
     Diagram of the thermal management system. Dynamic states are bolded. }
    \label{fig-TMS_Diagram}
\end{figure}

The proposed TMS architecture consists of five elements, a cold plate that was chosen to absorb a bounded heat load $\dot{Q}_{cp}$, a heat exchanger that rejects heat from the TMS to a secondary fluid at a rate of $\dot{Q}_{hx}$, a TES module that rejects heat from the working fluid to a PCM at a rate of $\dot{Q}_{TES}$, a water tank that stores thermal energy as sensible heat, and a pump that drives the primary mass flow rate. The system is modeled using eight dynamic states. The cold plate and heat exchanger are both modeled with two dynamic states, one for the temperature of the fluid contained within the control volume, denoted by $f$ in the subscript, and another for the temperature of the metal wall, denoted by $w$ in the subscript. Heat is exchanged between the two dynamic states through convection with a heat transfer coefficient $\alpha$ and contact surface area $A$. The resulting dynamic equations are given by
\begin{subequations}\label{eqn-TMSdynamics}
\begin{align}
    &C_{cp,w}\frac{dT_{cp,w}}{dt}=\alpha_{cp}A_{cp}(T_{cp,f}-T_{cp,w})+\dot{Q}_{cp}\:,\\
    &C_{cp,f}\frac{dT_{cp,f}}{dt}=\alpha_{cp}A_{cp}(T_{cp,w}-T_{cp,f})+c_p\dot{m}_p(T_{t,f}-T_{cp,f})\:,\\
    &C_{hx,w}\frac{dT_{hx,w}}{dt}=\alpha_{hx}A_{hx}(T_{hx,f}-T_{hx,w})-\dot{Q}_{hx}\:,\\
    &C_{hx,f}\frac{dT_{hx,f}}{dt}=\alpha_{hx}A_{hx}(T_{hx,w}-T_{hx,f})+c_p\dot{m}_p(T_{cp,f}-T_{hx,f})\:,
\end{align}
\end{subequations}
where $\dot{m}_p$ is the mass flow rate of the primary working fluid with specific heat $c_p$, and $\dot{Q}_{cp}$ is the heat load applied to the cold plate. The heat transfer rate between the primary and secondary fluids is modeled using the effectiveness-NTU method as
\begin{equation}
    \dot{Q}_{hx}=c_p\dot{m}_s(T_{s}-T_{hx,w})\left(\exp\left[\frac{-\alpha_{hx,s}A_{hx,s}}{c_p\dot{m}_s}\right]-1\right)
\end{equation}

. The cold plate is modeled using two states with dynamics described by 
\begin{subequations}\label{eqn-CP}
\begin{align}
    &C_{cp,w}\frac{dT_{cp,w}}{dt}=\alpha_{cp}A_{cp}(T_{cp,f}-T_{cp,w})+\dot{Q}_{cp}\:,\\
    &C_{cp,f}\frac{dT_{cp,f}}{dt}=\alpha_{cp}A_{cp}(T_{cp,w}-T_{cp,f})+c_p\dot{m}_p(T_{t,f}-T_{cp,f})\:,
\end{align}
\end{subequations}
where $T_{cp,w}$ is the temperature of the metal wall with thermal capacitance $C_{cp,w}$, $T_{cp,f}$ is the temperature of the fluid within the control volume with thermal capacitance $C_{cp,f}$, $T_{t,f}$ is the temperature of the fluid leaving the tank, $\dot{m}_p$ is the mass flow rate of the primary working fluid, $\dot{Q}_{cp}$ is the heat load applied to the cold plate, and the heat transfer rate between the two states is governed by the heat transfer coefficient $\alpha_{cp}$ and contact surface area $A_{cp}$. The dynamics of the heat exchanger is modeled using two states with dynamics described by
\begin{subequations}\label{eqn-HX}
\begin{align}
    &C_{hx,w}\frac{dT_{hx,w}}{dt}=\alpha_{hx}A_{hx}(T_{hx,f}-T_{hx,w})-\dot{Q}_{hx}\:,\\
    &C_{hx,f}\frac{dT_{hx,f}}{dt}=\alpha_{hx}A_{hx}(T_{hx,w}-T_{hx,f})+c_p\dot{m}_p(T_{cp,f}-T_{hx,f})\:,
\end{align}
\end{subequations}



The cold plate is modeled using 
